Bag of Tricks to Boost Adversarial Transferability

Deep neural networks are widely known to be vulnerable to adversarial examples. However, vanilla adversarial examples generated under the white-box setting often exhibit low transferability across different models. Since adversarial transferability poses more severe threats to practical applications, various approaches have been proposed for better transferability, including gradient-based, input transformation-based, and model-related attacks, \etc. In this work, we find that several tiny changes in the existing adversarial attacks can significantly affect the attack performance, \eg, the number of iterations and step size. Based on careful studies of existing adversarial attacks, we propose a bag of tricks to enhance adversarial transferability, including momentum initialization, scheduled step size, dual example, spectral-based input transformation, and several ensemble strategies. Extensive experiments on the ImageNet dataset validate the high effectiveness of our proposed tricks and show that combining them can further boost adversarial transferability. Our work provides practical insights and techniques to enhance adversarial transferability, and offers guidance to improve the attack performance on the real-world application through simple adjustments.

==> tabs/rgi_de.tex <==
\begin{table}[!ht]
    \label{tab:rgi_de}
    \centering
    \captionof{table}{Targeted attack performance against different models. Results with 300 iterations are reported. We denote RGI as the random gloabl initialization, and DE as the dual example strategy.}
    \begin{tabular}{ccccc}
    \toprule
        Method & DenseNet121 & VGG16 & Inception-v3 &  \\ \midrule
        Po+Trip & 54.7 & 34.4 & 5.9 &  \\ 
        RGI+Po+Trip & 58.6 & 37.2 & 8.3 &  \\
        DE+Po+Trip & 60.8 & 38.2 & 9.1 &  \\ 
        logit & 72.5 & 62.7 & 9.4 &  \\ 
        RGI+logit & 78.3 & 65.7 & 13.5 &  \\ 
        DE+logit & 77.4 & 65.2 & 12.7 & \\ \bottomrule
    \end{tabular}
\end{table}
